Data Sharing and Compression for Cooperative Networked Control

Sharing forecasts of network timeseries data, such as cellular or electricity load patterns, can improve independent control applications ranging from traffic scheduling to power generation. Typically, forecasts are designed without knowledge of a downstream controller's task objective, and thus simply optimize for mean prediction error. However, such task-agnostic representations are often too large to stream over a communication network and do not emphasize salient temporal features for cooperative control. This paper presents a solution to learn succinct, highly-compressed forecasts that are co-designed with a modular controller's task objective. Our simulations with real cellular, Internet-of-Things (IoT), and electricity load data show we can improve a model predictive controller's performance by at least $25\%$ while transmitting $80\%$ less data than the competing method. Further, we present theoretical compression results for a networked variant of the classical linear quadratic regulator (LQR) control problem.

==> sections/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
      \answerYes{\textbf{Please see Section \ref{sec:intro}.}}
  \item Did you describe the limitations of your work?
      \answerYes{\textbf{Please see the end of the evaluation (Section \ref{sec:evaluation}).}}
  \item Did you discuss any potential negative societal impacts of your work?
      \answerYes{\textbf{The work aims to provide positive societal impacts by optimizing social systems. We discussed privacy as a future step in Section \ref{sec:conclusion}.}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
      \answerYes{\textbf{Please see Section \ref{sec:algorithm}.}}
    \item Did you include complete proofs of all theoretical results?
        \answerYes{\textbf{Please see Section \ref{sec:algorithm}.}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
      \answerYes{\textbf{Please see Appendix Section \ref{sec:appendix_evaluation}.}}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerYes{\textbf{Please see the plots in Section 5.}}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \answerYes{\textbf{Please see Appendix Section \ref{sec:appendix_evaluation}.}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
      \answerYes{\textbf{Please see the citations for all three publicly-available datasets in Section \ref{sec:scenarios}.}} 
  \item Did you mention the license of the assets?
      \answerYes{\textbf{As stated in the Appendix, the licenses for the individual assets were not given online.}}
  \item Did you include any new assets either in the supplemental material or as a URL?
      \answerYes{\textbf{We provide our collected IoT dataset in the supplement and will make it publicly-available online.}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
      \answerYes{\textbf{Please see Appendix Section \ref{sec:appendix_evaluation}.}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
      \answerYes{\textbf{Yes, we stated in Appendix Section \ref{sec:appendix_evaluation} that there no is no personally identifiable or private information.}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

